FreeCHR: An Algebraic Framework for CHR-Embeddings

We introduce the framework FreeCHR which formalizes the embedding of Constraint Handling Rules (CHR) into a host language, using the concept of initial algebra semantics from category theory. We hereby establish a high-level implementation scheme for CHR as well as a common formalization for both theory and practice. We propose a lifting of the syntax of CHR via an endofunctor in the category Set and a lifting of the very abstract operational semantics of CHR into FreeCHR, using the free algebra, generated by the endofunctor. We give proofs for soundness and completeness w.r.t. its original definition. We also propose a first abstract execution algorithm and prove correctness w.r.t. the operational semantics. Finally, we show the practicability of our approach by giving two possible implementations of this algorithm in Haskell and Python. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> tex/sections/implementation_old.tex <==
\input{snippets/FreeCHR.hs.tex}
\input{snippets/FreeCHR.py.tex}

\section{Implementation case studies}\label{sec::freechr:instance:very-abstract:case-studies}

In this section, we want to introduce two example implementations of \autoref{alg::freechr:imp:set:alg:very-abstract} in Haskell and Python.
The full source code is available at GitHub \footnote{\textcolor{red}{(needs a new one)} \url{https://gist.github.com/SRechenberger/739683a23f8a9978ae601c6c815d61c4}}.
We want to discuss how the host language flavors FreeCHR instances and the practical implications of the flavoring, as well as how different instances compare to each other.

Both implementations do not strictly follow \autoref{alg::freechr:imp:set:alg:very-abstract} as they lack the non-determinism.
One can easily see, though, that they only perform valid transitions by comparing them to \autoref{alg::freechr:imp:set:alg:very-abstract}

They will also not account for trivial non-termination due to repeated application of propagation rules,
since a rule might be applied repeatedly to the same constraints.
In CHR this is solved by recording a \emph{propagation history} as supported by the \emph{abstract} operational semantics described in \cite{fruehwirth2009constraint}.
An implementation supporting this can also be found on GitHub \footnote{\textcolor{red}{URL}}.
As a consequence, the presented implementations effectively model only a subset of CHR without propagation rules.
Also, the matching algorithms are very naive and will not perform very well.

\subsection{Implementation in Haskell}
We will first discuss the Haskell implementation.
This can be viewed as an example of an instance in a pure functional language with a very strict and static type system.
Since modern languages tend to adopt more and more functional features (see \EG Kotlin and Java), many aspects discussed here will be relevant for other host languages as well.

\subsubsection{Carrier}
For this implementation the type \haskell{SolverStep c}, which can be seen in \autoref{fig::impl:solver:hs}, implements the carrier of the algebra.
It is parameterized over the type of constraints.
The value of this type is essentially equivalent to a plain function of type \haskell{[c] -> [c]}, but wrapping them allows the implementation of type class instances.
This way, we can also discern a FreeCHR program which is \emph{"in construction"} from one that was processed by \textsc{run}, preventing accidental mixing which might cause issues.

An important difference of this, as well as the Python implementation, to the algorithms presented in \autoref{sec::freechr:instance:very-abstract} is that they use lists instead of multisets, removing an element of non-determinism.

\begin{figure}[t]
  \snippetHSsolverStep[firstnumber=1]
  \caption{Wrapped solver function type}
  \label{fig::impl:solver:hs}
\end{figure}

\subsubsection{Execution algorithm}
The \haskell{rule} function can be seen in \autoref{fig::impl:rule:hs}.
The imposed constraint \haskell{Eq} on constraints is necessary to remove constraints from the state.
The function generates a new \haskell{SolverStep} object and works as follows:
First, it is attempted to find a matching (l. 5), for which the guard is satisfied.
A matching is naively computed by the function \haskell{match}, which can be seen in \autoref{fig::impl:match:hs}.
It lazily computes a list of all permutations (l. 5) of all subsequences with the same length as the head of the rule (l. 3 and 4) and checks whether the elements of the sequence satisfy the respective predicate in the head (l. 6).
If such a matching is found it is passed to the body of the rule.
The expression in line 7 corresponds to the return value in line \ref{alg::freechr:imp:set:alg:very-abstract:2} of \autoref{alg::freechr:imp:set:alg:very-abstract}.

\begin{figure}[t]
  \snippetHSrule[firstnumber=1]
  \caption{Haskell implementation of \textsc{rule}}
  \label{fig::impl:rule:hs}
\end{figure}


\begin{figure}[t]
  \snippetHSmatch[firstnumber=1]
  \caption{Haskell implementation of matching}
  \label{fig::impl:match:hs}
\end{figure}


The implementation of \textsc{compose} can be seen in \autoref{fig::impl:compose:hs}.
It is implemented by interpreting the type \haskell{SolverStep} as a Semigroup and implementing its binary operation \haskell{(<>)}. Hence, \textsc{compose} is always interpreted as an associative binary operator.
Again, there is an \haskell{Eq} constraint imposed on the type of constraints.
This time, it is used to compare states to discern whether the first subprogram changes the state (l. 6).
If this is not the case, the second is tried (l. 7), otherwise the state is returned (l. 8).

Here, the non-determinism of the abstract \textsc{compose} implementation is solved by trying the subprograms of an expression \haskell{p1 <> p2 <> ... <> pn} from left to right.
\begin{figure}[t]
  \snippetHScompose[firstnumber=1]
  \caption{Haskell implementation of \textsc{compose}}
  \label{fig::impl:compose:hs}
\end{figure}

The \textsc{run} function is implemented as in \autoref{fig::impl:run:hs}.
Analously to \autoref{alg::freechr:imp:set:alg:run} it first applies the program to the state (l. 6).
It then checks, whether the result is equal to the input.
If this is the case, the state is returned (l. 3).
Otherwise, \haskell{run} calls itself with the new state (l. 4).

\begin{figure}[t]
  \snippetHSrun[firstnumber=1]
  \caption{Haskell implementation of \textsc{run}}
  \label{fig::impl:run:hs}
\end{figure}

\subsubsection{Features and Issues}
The Haskell implementation is very true to the functional nature of the definition of FreeCHR.
It provides the instances with free type checking and tight control over the behavior of programs.
On the other hand, as we can see in, \EG \autoref{fig::impl:gcd:hs} it can be somewhat verbose.
We have to explicitly match on lists in the functions for guard and body.
This might be avoidable with some functional trickery, though.

\begin{figure}[t]
  \snippetHSgcd[firstnumber=1]
  \caption{Greatest Common Divisor in FreeCHR(Haskell)}
  \label{fig::impl:gcd:hs}
\end{figure}

\iffalse
\begin{figure}[t]
  \snippetHSfib[firstnumber=1]
  \caption{Fibonacci numbers in FreeCHR(Haskell)}
  \label{fig::impl:fib:hs}
\end{figure}

\begin{figure}[t]
  \snippetHSnub[firstnumber=1]
  \caption{Removing duplicates in FreeCHR(Haskell)}
  \label{fig::impl:nub:hs}
\end{figure}
\fi


\subsection{Implementation in Python}
Next, we will discuss a FreeCHR instance implemented in Python.
Python is a popular example of a dynamically typed imperative language.

\subsubsection{Execution Algorithm}
To implement the currying the abstract definition of FreeCHR made heavy use of, the Python implementation of \textsc{rule}, which can be seen in \autoref{fig::impl:rule:py}, returns merely a function that performs the actual work.

\begin{figure}[t]
  \snippetPYrule[firstnumber=1]
  \caption{Python implementation of \textsc{rule}}
  \label{fig::impl:rule:py}
\end{figure}

The function \python{solver} (l. 3) accepts the state as a sequence of constraints.
It first, as above, tries to find a sequence of matching constraints.
Again, matchings are computed lazily, this time via iterators (see \autoref{fig::impl:match:py}).
If no such sequence is found, the function returns the state unaltered (l. 8).
Otherwise, to keep the original input unchanged a copy is created.
From this copy, all constraints contained in the part of the matching matched to the removed head are removed from the new state (Lines 11 and 12).
Then, again, the matching is passed to the body of the rule and the resulting list is added to the new state (l. 14).

\begin{figure}[t]
  \snippetPYmatch[firstnumber=1]
  \caption{Python implementation of matching}
  \label{fig::impl:match:py}
\end{figure}


The implementation of \textsc{compose} (\autoref{fig::impl:compose:py}), also merely defines and returns a function.
It accepts the state as a sequence of values and iterates over the subprograms (\python{*solvers}), passed to \python{compose}.
As soon as a subprogram that alters the state is found, the loop will be interrupted (l. 6 and 7) and the altered state returned (l. 9).

\begin{figure}[t]
  \snippetPYcompose[firstnumber=1]
  \caption{Python implementation of \textsc{compose}}
  \label{fig::impl:compose:py}
\end{figure}

The implementation of \textsc{run} as seen in \autoref{fig::impl:run:py} receives the program and returns a function, that will apply it to the state as long as this alters it.

\begin{figure}[t]
  \snippetPYrun[firstnumber=1]
  \caption{Python implementation of \textsc{run}}
  \label{fig::impl:run:py}
\end{figure}

\subsubsection{Features and Issues}
The implementation does make heavy use of the spread operator provided by Python, especially to add convenience in usage, as can be seen in \autoref{fig::impl:gcd:py}, when compared to the Haskell implementation of \autoref{fig::impl:gcd:hs}.
The matched constraints are spread when passed to the guard and the body (\autoref{fig::impl:rule:py}, l. 5 and 14), which allows to write the respective functions more naturally.

\begin{figure}[t]
  \snippetPYgcd[firstnumber=1]
  \caption{Greatest Common Divisor in FreeCHR(Python)}
  \label{fig::impl:gcd:py}
\end{figure}

On the downside, Python does not allow for statements in anonymous functions, \IE more complex guards and bodies need to be defined separately, as seen in \autoref{fig::impl:alldiff:py}.
This is a common problem in all host languages that do not at all or not sufficiently support anonymous functions, like, \EG C.

\begin{figure}[t]
  \snippetPYalldiff[firstnumber=1]
  \caption{Implementation of \texttt{all\_diff} constraint in FreeCHR(Python)}
  \label{fig::impl:alldiff:py}
\end{figure}

The program in \autoref{fig::impl:alldiff:py} shows another aspect encountered in host languages that do, unlike Haskell, not explicitly handle side effects.
The rule will raise an \python{Exception} if it fires.
If not prohibited by the host language, arbitrary side effects may be caused and influence the execution of FreeCHR program. 
This is not covered by the operational semantics, yet.
If mindfully used, this can be used anyway, though, especially for logging and debugging.

\subsection{Summary}
As demonstrated in the case studies the abstract execution algorithms serve as a viable guideline to implement the embedded FreeCHR language.
The user has to take care, though.
FreeCHR will be heavily flavored by the host language and will possibly allow for undefined behavior.
If mindfully used, though, this already allows for some practical use of FreeCHR.



==> tex/sections/instances.tex <==
\section{Instances}\label{sec::freechr:instance}

Since the $\omstara$ operational semantics define the execution of FreeCHR programs as a state transition system, an obvious way to implement FreeCHR is by mapping programs to functions mappings a state to its successor.


\begin{definition}[FreeCHR instance]
  An \emph{instance} of FreeCHR is a $\chr_C$-algebra
  \begin{align*}
    \left((\fmultiset C)^{\fmultiset C}, \left[\chrinstrule, \chrinstcomp\right] \right)
  \end{align*}
  with
  \begin{align*}
    \chrinstrule &: \flist \tbool^C \setprod \flist \tbool^C \setprod \tbool^{\flist C} \setprod \left(\fmultiset C\right)^{\flist C} \longrightarrow (\fmultiset C)^{\fmultiset C}\\
    \chrinstcomp &: (\fmultiset C)^{\fmultiset C} \setprod (\fmultiset C)^{\fmultiset C} \longrightarrow (\fmultiset C)^{\fmultiset C}
  \end{align*}
\end{definition}

A FreeCHR instance hence needs to define the two functions $\chrinstrule$ and $\chrinstcomp$ which implement the execution of programs and hence the operational semantics of the program.
$\chrinstrule$ implements the application of a single rule to a state if it is possible. $\chrinstcomp$ implements the execution strategy of, fundamentally, a sequence of rules to a state.
Both are only concerned with single execution steps.
We hence also need the function
\begin{align*}
  \mathtt{run} : (\fmultiset C)^{\fmultiset C} \longrightarrow (\fmultiset C)^{\fmultiset C}
\end{align*}
which maps a function performing singular steps to a function applying this function until a final state is reached. In CHR this generally means, until no rules can be applied to the state.

Since an instance practically also defines operational semantics it makes sense to directly associate it with an LTS as well.
\begin{definition}[LTS of a FreeCHR instance]\label{def::freechr:instance-rel}
  Let
  \begin{align*}
    I = \left((\fmultiset C)^{\fmultiset C}, \left[\rho, \nu\right]\right) 
  \end{align*}
  $I$ implies an LTS
  \begin{align*}
    \trrel I = \langle \fmultiset C, L, \mapsto\rangle
  \end{align*}
  where the labels $L$ are recursively defined as
  \begin{align*}
    L =& \left\{\rho(k, r, g, b) \mid k, r \in \flist (\tbool^C), g \in \tbool^{\flist C}, b \in (\fmultiset C)^{\flist C}\right\}
      \cup \left\{\nu(f, g) \mid f, g \in L \right\}
  \end{align*}
  and the transition relation as
  \begin{align*}
    (\mapsto) =& \left\{s \xmapsto{f} s' \mid s \in \fmultiset C, f \in L, f(s) \equiv_{\fmultiset C} s'\right\}
  \end{align*}
\end{definition}

With this, we can easily verify an instance against operational semantics, using the concepts from \autoref{sec::lts}.
We will do so from the perspective of the operational semantics, instead of from the perspective of the implementation.
To verify, that an instance only performs valid transitions, we hence prove \emph{$\fembed$-completeness}
\begin{align*}
  S \freetr{p} S' \Longleftarrow S \freetr{\kata{\alpha}(p)} S'
\end{align*}
Consequently, to prove that the implementation can perform all valid transitions, we prove \emph{$\fembed$-soundness up to repeated transition}
\begin{align*}
  S \freetr{p} S' \Longrightarrow S \xmapsto{\kata{\alpha}(p)}^{*} S'
\end{align*}
We need the relaxation \emph{"up to repeated transition"} since the instances, and hence their respective LTS, are only defined for singular steps.

